Nonequilibrium relaxation of a trapped particle in a near-critical Gaussian field

We study the non-equilibrium relaxational dynamics of a probe particle linearly coupled to a thermally fluctuating scalar field and subject to a harmonic potential, which provides a cartoon for an optically trapped colloid immersed in a fluid close to its bulk critical point. The average position of the particle initially displaced from the position of mechanical equilibrium is shown to feature long-time algebraic tails as the critical point of the field is approached, the universal exponents of which are determined in arbitrary spatial dimensions. As expected, this behavior cannot be captured by adiabatic approaches which assume fast field relaxation. The predictions of the analytic, perturbative approach are qualitatively confirmed by numerical simulations.

==> Pgfplots/ModelA.tex <==
% Data was obtained with
% NIntegrate[...,  
%   Method -> "LobattoKronrodRule",
%   WorkingPrecision -> 10 ~ 15,
%   Maxpoints -> 5*10^4 ~ 5*10^5]
% 

% Data load
\pgfplotstableread{ModelA-dim1.txt}{\modelAdimOne}
\pgfplotstableread{ModelA-dim2.txt}{\modelAdimTwo}
\pgfplotstableread{ModelA-dim3.txt}{\modelAdimThree}

% Axis style
\pgfplotsset{
    modelA_axis/.style = {
        height = 0.29\textwidth,
        each nth point = 2, 
        xmin = 1, xmax = 10^4,
        xtick = {1, 10.1, 10^2, 10^3, 10^4},
        ymin = 10^-9, ymax=10,
        ytick = {1, 10^-3, 10^-6, 10^-9},
        minor tick num = 0,
        xtick pos = lower,
        ytick pos = left,
        % max space between ticks = 20,
        tick style = {black},
        xlabel = $\gamma t$,
        % ylabel = $\langle{X(t)}\rangle$,
        cycle list name = modelA_marks,
        mark size = 1.3 pt,
        clip marker paths=true, axis on top=true,
    }
}

% Legend style
\pgfplotsset{
    modelA_legend/.style = {
        legend entries = {
            $Dr/\nu k = 1$,
            $Dr/\nu k = 10^{-1}$,
            $Dr/\nu k = 10^{-2}$,
            $Dr/\nu k = 0$
        },
        legend columns = -1, % landscape legend
        legend to name = legendA, % to put the legend outside
        legend style = {
            text=black,
            /tikz/every even column/.append style={column sep=0.5cm}},
    }
}
  
% Point styles 
\pgfplotscreateplotcyclelist{modelA_marks} {
    {cyan,mark=*},
    {orange,mark=square*},
    {teal,mark=triangle*},
    {red,mark=diamond*}
}

{\scalefont{1}\centering%
\tikzsetnextfilename{ModelA-dim1}%
\begin{tikzpicture}
    \begin{loglogaxis} [
            modelA_axis, modelA_legend,
            title={$d=1$},
            ylabel = $\langle{X(t)}\rangle$,
        ]
        %% only lambda^2 correction:
        % \addplot table[x=t, y=r01]   {\modelAdimOne};
        % \addplot table[x=t, y=r001]  {\modelAdimOne};
        % \addplot table[x=t, y=r0001] {\modelAdimOne};
        % \addplot table[x=t, y=r0]    {\modelAdimOne};

        %% e^(-nu*k*t) + lambda^2*correction
        \addplot table[x=t, y expr={\AddFreeTen{r1}}]   {\modelAdimOne};
        \addplot table[x=t, y expr={\AddFreeTen{r01}}]  {\modelAdimOne};
        \addplot table[x=t, y expr={\AddFreeTen{r001}}] {\modelAdimOne};
        \addplot table[x=t, y expr={\AddFreeTen{r0}}]   {\modelAdimOne};
        \addplot[domain = 300:10^6] {80*x^(-3/2)};
        \node at (axis cs:2*10^3,20*10^-3) [anchor=center] {$t^{-3/2}$};
    \end{loglogaxis} 
\end{tikzpicture}~%
\tikzsetnextfilename{ModelA-dim2}%
\begin{tikzpicture}
    \begin{loglogaxis}[
            modelA_axis,
            title={$d=2$}, 
            % yticklabels = {},
        ]
        % \addplot table[x=t, y=r01]   {\modelAdimTwo};
        % \addplot table[x=t, y=r001]  {\modelAdimTwo};
        % \addplot table[x=t, y=r0001] {\modelAdimTwo};
        % \addplot table[x=t, y=r0]    {\modelAdimTwo};

        \addplot table[x=t, y expr={\AddFreeTen{r1}}]   {\modelAdimTwo};
        \addplot table[x=t, y expr={\AddFreeTen{r01}}]  {\modelAdimTwo};
        \addplot table[x=t, y expr={\AddFreeTen{r001}}] {\modelAdimTwo};
        \addplot table[x=t, y expr={\AddFreeTen{r0}}]    {\modelAdimTwo};
        \addplot[domain = 300:10^6] {25*x^(-2)};
        \node at (axis cs:2*10^3, 15*10^-5) [anchor=center] {$t^{-2}$};
    \end{loglogaxis} 
\end{tikzpicture}~%
\tikzsetnextfilename{ModelA-dim3}%
\begin{tikzpicture}
    \begin{loglogaxis} [
            modelA_axis,
            title={$d=3$},
            % yticklabels={},
        ]
        % \addplot table[x=t, y=r01]   {\modelAdimThree};
        % \addplot table[x=t, y=r001]  {\modelAdimThree};
        % \addplot table[x=t, y=r0001] {\modelAdimThree};
        % \addplot table[x=t, y=r0]    {\modelAdimThree};
    
        \addplot table[x=t, y expr={\AddFreeTen{r1}}]   {\modelAdimThree};
        \addplot table[x=t, y expr={\AddFreeTen{r01}}]  {\modelAdimThree};
        \addplot table[x=t, y expr={\AddFreeTen{r001}}] {\modelAdimThree};
        \addplot table[x=t, y expr={\AddFreeTen{r0}}]    {\modelAdimThree};

        \addplot[domain = 300:10^6] {8*x^(-5/2)};
        \node at (axis cs:2*10^3,4*10^-6) [anchor=center] {$t^{-5/2}$};
    \end{loglogaxis} 
\end{tikzpicture}\\%
\ref{legendA}
}

==> Pgfplots/ModelB.tex <==
% Data was obtained with
% NIntegrate[..., 
%   Method -> "LobattoKronrodRule", 
%   MaxPoints -> 5*10^4 / 5*10^4 / 10^5,
%   WorkingPrecision -> 10 / 10 / 20]

% Data load
\pgfplotstableread{ModelB-dim1.txt}{\modelBdimOne}
\pgfplotstableread{ModelB-dim2.txt}{\modelBdimTwo}
\pgfplotstableread{ModelB-dim3.txt}{\modelBdimThree}

% Axis style
\pgfplotsset
    {modelB_axis/.style= {
        height = 0.29\textwidth,
        each nth point = 2, 
        xmin = 1, xmax = 10^4,
        ymin = 10^-10, ymax=1,
        max space between ticks = 20,
        tick style = {black},
        xtick pos = lower,
        ytick pos = left,
        xtick = {1, 10.1, 10^2, 10^3, 10^4},
        % xticklabels = {10^0, 10^1, 10^2, 10^3, 10^4},
        ytick = {1, 10^-3, 10^-6, 10^-9},
        xlabel = $\gamma t$,
        cycle list name = modelB_marks,
        mark size = 1.1 pt,
        clip marker paths=true, axis on top=true,
    }
}
   
% Legend style
\pgfplotsset{
    modelB_legend/.style = {
        legend entries = {
            $Dr^2/\nu k = 10$,
            $Dr^2/\nu k = 1$,
            $Dr^2/\nu k = 10^{-1}$,
            $Dr^2/\nu k = 0$
        },
        legend columns = -1, % landscape legend
        legend to name = legendB, % to put the legend outside
        legend style = {
            text=black,
            /tikz/every even column/.append style={column sep=0.5cm}},
    }
}

% Point styles 
\pgfplotscreateplotcyclelist{modelB_marks} {
    {cyan,mark=*},
    {orange,mark=square*},
    {teal,mark=triangle*},
    {red,mark=diamond*}
}

{\scalefont{1}\centering%
\tikzsetnextfilename{ModelB-dim1}%
\begin{tikzpicture}
    \begin{loglogaxis} [
            modelB_axis,
            modelB_legend,
            title={$d=1$},
            ylabel = $\langle{X(t)}\rangle$,
        ]
        %% only lambda^2 correction:
        % \addplot table[x=t, y=r10] {\modelBdimOne};
        % \addplot table[x=t, y=r1]  {\modelBdimOne};
        % \addplot table[x=t, y=r01] {\modelBdimOne};
        % \addplot table[x=t, y=r0]  {\modelBdimOne};

        %% e^(-nu*k*t) + lambda^2*correction
        \addplot table[x=t, y expr={\AddFree{r10}}] {\modelBdimOne};
        \addplot table[x=t, y expr={\AddFree{r1}}]  {\modelBdimOne};
        \addplot table[x=t, y expr={\AddFree{r01}}] {\modelBdimOne};
        \addplot table[x=t, y expr={\AddFree{r0}}]  {\modelBdimOne};

        \addplot[domain = 300:10^6] {3*10^(-1)*x^(-5/4)};
        \node at (axis cs:1*10^3,7*10^-4) [anchor=center] {$t^{-5/4}$};
        
        \addplot[domain = 50:10^6] {12*10^(-4)*x^(-5/2)};
        \node at (axis cs:30,4*10^-9) [anchor=center] {$t^{-5/2}$};
    \end{loglogaxis} 
\end{tikzpicture}~%
\tikzsetnextfilename{ModelB-dim2}%
\begin{tikzpicture}
    \begin{loglogaxis} [
            modelB_axis,
            title={$d=2$},
            % yticklabels = {},
        ]
        % \addplot table[x=t, y=r10] {\modelBdimTwo};
        % \addplot table[x=t, y=r1]  {\modelBdimTwo};
        % \addplot table[x=t, y=r01] {\modelBdimTwo};
        % \addplot table[x=t, y=r0]  {\modelBdimTwo};

        \addplot table[x=t, y expr={\AddFree{r10}}] {\modelBdimTwo};
        \addplot table[x=t, y expr={\AddFree{r1}}]  {\modelBdimTwo};
        \addplot table[x=t, y expr={\AddFree{r01}}] {\modelBdimTwo};
        \addplot table[x=t, y expr={\AddFree{r0}}]  {\modelBdimTwo};

        \node at (axis cs:1*10^3,4*10^-5) [anchor=center] {$t^{-3/2}$};
        \addplot[domain = 300:4*10^6] {8*10^(-2)*x^(-3/2)};
        
        \node at (axis cs:10^1,4*10^-9) [anchor=center] {$t^{-3}$};
        \addplot[domain = 20:10^6] {4*10^(-4)*x^(-3)};
    \end{loglogaxis}
\end{tikzpicture}~%
\tikzsetnextfilename{ModelB-dim3}%
\begin{tikzpicture}
    \begin{loglogaxis} [
            modelB_axis,
            title = {$d=3$},
            % yticklabels = {}
        ]
        % \addplot table[x=t, y=r10] {\modelBdimThree};
        % \addplot table[x=t, y=r1]  {\modelBdimThree};
        % \addplot table[x=t, y=r01] {\modelBdimThree};
        % \addplot table[x=t, y=r0]  {\modelBdimThree};
        
        \addplot table[x=t, y expr={\AddFree{r10}}] {\modelBdimThree};
        \addplot table[x=t, y expr={\AddFree{r1}}]  {\modelBdimThree};
        \addplot table[x=t, y expr={\AddFree{r01}}] {\modelBdimThree};
        \addplot table[x=t, y expr={\AddFree{r0}}]  {\modelBdimThree};

        \addplot[domain = 300:10^6] {20*10^(-3)*x^(-7/4)};
        \node at (axis cs:1*10^3,2*10^-6) [anchor=center] {$t^{-7/4}$};
        
        \addplot[domain = 10:10^6] {4*10^(-5)*x^(-7/2)};
        \node at (axis cs:4,4*10^-9) [anchor=center] {$t^{-7/2}$};
    \end{loglogaxis} 
\end{tikzpicture} \\%
\ref{legendB}
}

==> Pgfplots/Potential1.tex <==
% Point styles 
\pgfplotscreateplotcyclelist{Potential1_marks} {
    {cyan,mark=*},
    {orange,mark=square*},
    {teal,mark=triangle*},
    {red,mark=diamond*}
}

\tikzsetnextfilename{Potential1}%
\begin{tikzpicture}
    \begin{loglogaxis} [
            width = \columnwidth,
            height = 0.7\columnwidth,
            % width = \textwidth,
            each nth point = 2, 
            xmin = 1, xmax = 10^4,
            ymin = 10^-9, ymax = 10^0,
            xtick = {1, 10.1, 10^2, 10^3, 10^4},
            ytick = {1, 10^-3, 10^-6, 10^-9},
            tick style = {black},
            xtick pos = lower,
            ytick pos = left,
            xlabel = $\gamma t$,
            ylabel = $\langle{X(t)}\rangle$,
            cycle list name = Potential1_marks,
            mark size = 1.5pt,
            clip marker paths=true, axis on top=true,
            legend entries = {
                $n=0$, $n=2$, $n=4$,
            },
            legend style = {text = black},
            legend pos = north east,
        ]
        \addplot table[x=t, y expr={\AddFree{n0}}] {Potential1.txt};
        \addplot table[x=t, y expr={\AddFree{n2}}] {Potential1.txt};
        \addplot table[x=t, y expr={\AddFree{n4}}] {Potential1.txt};
        
        \addplot[domain = 300:10^5] {0.5*x^(-3/2)};
        \node at (axis cs:2*10^3,10^-4) [anchor=center] {$t^{-3/2}$};
        
        \addplot[domain = 70:10^5] {2*x^(-7/2)};
        \node at (axis cs:3*10^2,10^-7) [anchor=center] {$t^{-7/2}$};
        
        \addplot[domain = 20:10^5] {1.5*x^(-11/2)};
        \node at (axis cs:10,10^-8) [anchor=center] {$t^{-11/2}$};
    \end{loglogaxis} 
\end{tikzpicture}

==> Pgfplots/Potential2.tex <==
% Point styles 
\pgfplotscreateplotcyclelist{Potential2_marks} {
    {cyan,mark=*},
    {orange,mark=square*},
    {teal,mark=triangle*},
    {red,mark=diamond*}
}

\tikzsetnextfilename{Potential2}%
\begin{tikzpicture}
    \begin{loglogaxis} [
            % width = 0.32\textwidth,
            width = \columnwidth,
            height = 0.7\columnwidth,
            each nth point = 3, 
            xmin = 1, xmax = 100,
            ymin = 10^-4, ymax = 10^-1,
            xtick = {1, 10.1, 100},
            ytick = {1, 0.1, 10^-2, 10^-3, 10^-4},
            max space between ticks = 20,
            tick style = {black},
            xtick pos = lower,
            ytick pos = left,
            xlabel = $\gamma t$,
            ylabel = $\langle{X\2(t)}\rangle$,
            cycle list name = Potential2_marks,
            mark size = 1.5 pt,
            clip marker paths=true, axis on top=true,
            legend entries = {Gaussian, Box, Cusp},
            legend style = {text = black},
        ]
        \addplot table[x=t, y=gaussian] {Potential2.txt};
        \addplot table[x=t, y=box] {Potential2.txt};
        \addplot table[x=t, y=cusp] {Potential2.txt};
        \addplot[domain = 20:100] {0.25*x^(-3/2)};
        \node at (axis cs:60,0.0015) [anchor=center] {$t^{-3/2}$};
    \end{loglogaxis} 
\end{tikzpicture}
